Spectral Galerkin methods for transfer operators in uniformly expanding dynamics

Markov expanding maps, a class of simple chaotic systems, are commonly used as models for chaotic dynamics, but existing numerical methods to study long-time statistical properties such as invariant measures have a poor trade-off between computational effort and accuracy. We develop a spectral Galerkin method for these maps' transfer operators, estimating statistical quantities using finite submatrices of the transfer operators' infinite Fourier or Chebyshev basis coefficient matrices. Rates of convergence of these estimates are obtained via quantitative bounds on the full transfer operator matrix entries; we find the method furnishes up to exponentially accurate estimates of statistical properties in only a polynomially large computational time. To implement these results we suggest and demonstrate two algorithms: a rigorously-validated algorithm, and a fast, more convenient adaptive algorithm. Using the first algorithm we prove rigorous bounds on some exemplar quantities that are substantially more accurate than previous. We show that the adaptive algorithm can produce double floating-point accuracy estimates in a fraction of a second on a personal computer.

==> Spectral-setup.tex <==
\subsection{Systems under consideration}\label{ss:setup}

In this section we will first introduce the two classes of chaotic maps that we will consider in the paper: one defined on periodic intervals, and one defined on non-periodic intervals. We will then introduce and discuss some generalised distortion conditions that maps in these classes may optionally satisfy and which determine the %. The satisfaction of these generalised distortion conditions determines the 
rate of convergence of spectral approximations. 

\subsubsection{Maps on periodic domains}

The first class $\upd$ we consider will be $C^2$ circle maps $f$ on the canonical periodic interval $[0,2\pi)$, satisfying the uniform expansion condition
	\begin{equation} \lambda := \inf_{x\in[\Lambda)} |f'(x)| > 1, \label{ue_definition}\tag{E}\end{equation}
and having bounded distortion
\cite{Gouezel14, Galatolo14, DeMelo12}:
%\begin{equation} \sup_{x\in[-1,1], \iota \in I} \left|\frac{v_\iota''(x)}{v_\iota'(x)}\right| < \infty.\tag{$\DD_1$}\label{distortion_basic}\end{equation}
\begin{equation} \sup_{x\in[\Lambda)} \left|\frac{f''(x)}{f'(x)^2}\right| < \infty.\tag{$\DD_1$}\label{distortion_basic}\end{equation}

	We will treat the inverses of maps in $\upd$ using lifts. The definition of $\upd$ implies that $f \in \upd$ can be lifted to a map $\hat f$ from $[0,2\pi)$ to the periodic interval $[0,2\beta \pi)$, where
	\[ \beta = \frac{1}{2\pi} \left| \int_0^{2\pi} f'(x) dx \right| \in \N^+. \]
	The lift $\hat f$ is a bijection, with inverse map $v: [0,2\beta\pi) \to [0,2\pi)$. This is illustrated in Figure \ref{f:setup}(a).
	For consistency with the maps defined in the next section, we also use the notation $v_\iota(x) = v(x+2\iota \pi)$ for $x\in[0,2\pi]$, $\iota \in I := \{0,1,\ldots,\beta-1\}$.
	
	
	\begin{figure}[htbp]
		\centering
		\includegraphics[width=\linewidth]{figures/setup}
		\caption{In (a), an example of a map $f \in \upd$ (yellow line) with its lift $\hat f$ (red dashes).
			In (b), an example of a map $f \in \unp$ (black) with branches indexed by $I = \{p,q,r\}$. Branches of the map $\hat f_\iota$ (cyan, pink, yellow dashes) are illustrated with their branch domains $\O_\iota$.} %and its branches $\hat f_\iota$ on their domains of definition .}
		\label{f:setup}
	\end{figure}
	
\subsubsection{Maps on non-periodic domains}

The second major class $\unp$ are full-branch Markov maps defined on the non-periodic interval $\Lambda = [-1,1]$. These may have possibly a countably infinite number of branches. %There are four conditions upon them, which we will state here and then discuss: 
%We say that there exists a set of closed intervals $\O_\iota$ for $\iota$ in some index set $I$ such that the interiors of the $\O_\iota$ partition a set $\Lambda^* \subset [-1,1]$ of full measure and each restriction $f|_{\intr \O_\iota}$ may be extended to a $C^2$ bijection $\hat f_\iota : \O_\iota \to [-1,1]$. 
We denote the extension of the $f |_{\O_\iota}$ to $ \overline{\O_\iota}$ by $\hat f_\iota: \overline{\O_\iota} \to \Lambda$ and require that these are at least $C^2$. A map of this kind is illustrated in Figure \ref{f:setup}(b).

We denote the branches of the inverse of $f$ by of $ v_\iota := \hat f_\iota^{-1}: [-1,1] \to \overline{\O_\iota}$.

Maps in $\unp$ must satisfy three further conditions. Firstly as with maps in $\unp$ they must satisfy bounded distortion condition (\ref{distortion_basic}), which may be reformulated as
\begin{equation} \sup_{x\in[-1,1], \iota \in I} \left|\frac{v_\iota''(x)}{v_\iota'(x)}\right| < \infty.\tag{$\DD_1$}.\end{equation}

To control high oscillatory behaviour of spectral basis functions near the endpoints of the interval we also introduce the {\it uniform C-expansion condition}: a map $f: [-1,1]\to [-1,1]$ is {\it uniformly C-expanding} if its associated {\it C-expansion parameter}
	\begin{equation} \check\lambda = \inf_{x\in\cup{\iota\in I} \O_\iota} \frac{\sqrt{1-x^2}}{\sqrt{1-f(x)^2}} |f'(x)| > 1. \tag{CE} \label{aue_definition} \end{equation}
This is equivalent to requiring $\cos\circ f\circ \cos^{-1}$ being uniformly-expanding with parameter $\check{\lambda}>1$.

When one restricts to Markov maps obeying (\ref{distortion_basic}), uniform C-expansion is, in effect, just uniform expansion. In particular, for every C-expanding $f$, all iterates $f^n$ for $n$ sufficiently large are uniformly expanding. Proofs and further discussion of C-expansion can be found in \ref{a:expanding-conjugacy}.%. Moreover, analytic conjugacies may be constructed from any given C-expanding (resp. expanding) map to some map in the other expansion category. Proofs and further discussion of C-expansion can be found in \ref{a:expanding-conjugacy}.

Finally, because of the singular $x = \cos\theta$ transformation from Fourier series to Chebyshev series, we will also introduce a constraint on maps in $\unp$ regarding the size and position of the branch domain intervals $\O_\iota$. This {\it partition spacing condition} requires that
\begin{equation} \sup\left\{ \frac{|\O_\iota|}{d(\O_\iota,\sigma)} : \iota \in I, \sigma \in \partial \Lambda, \sigma \notin \O_\iota \right\} = \Xi < \infty. \label{ppc}\tag{P}\end{equation}
If $|I|< \infty$, this condition is trivially satisfied. % unless there are an infinite number of branches clustered near the boundary of the interval. %; it only comes into play in an auxilliary lemma for Theorem \ref{t:entry_p}. 
%The partition spacing condition and its associated partition spacing constant $\Xi$ behave similarly to distortion bounds: for example constants, partition spacing constants of iterates of expanding maps are uniformly bounded. Such properties are outlined and proven in \ref{as:ppc}.

\subsubsection{Non-expanding maps}\label{sss:non-expanding}

We further consider maps that satisfy all the conditions of $\upd$ (resp. $\unp$) but for which the associated expansion parameters (\ref{ue_definition}) (resp. (\ref{aue_definition})) are merely positive, rather than strictly greater than one. These maps have similar structure to those in $\upd$ (resp. $\unp$), except that their dynamics are not necessarily chaotic. We denote the class of such maps $\bupd$ (resp. $\bunp$).

\subsubsection{Distortion conditions}

To obtain good convergence results we will optionally impose the following generalised distortion conditions on our maps. These generalised distortion conditions are equivalent to uniform bounds on derivatives of the distortion $\log |v_\iota'|$. %(see \ref{a:distortion} and 


%There are three families of regularity assumptions in $\D$: (\ref{distortion_diff_frac}) for $r \in \N^+$ and (\ref{distortion_ana_four},\ref{distortion_ana_cheb}) for $\delta > 0$. These are associated respectively with higher order differentiability and analyticity on periodic and non-periodic intervals, and imply these respective differential conditions; when the number of branches of $f^{-1}$ is finite, they are also implied by these conditions.

The first family of generalised distortion conditions are of the form %parametrised by $r \in \N^+$, and are comparable to (and slightly stronger than) $r+1$-times differentiability:
\begin{equation} \label{distortion_diff_frac}  \sup_{\iota\in I,x\in\Lambda}\left|\frac{v_\iota^{(n+1)}(x)}{v_\iota'(x)}\right|= C_n < \infty,\ n\leq r, \tag{$\DD_r$} \end{equation}
for $r \in \N^+$.
Note that the first of these conditions (\ref{distortion_basic}) is definitionally satisfied by maps in $\upd$ and $\unp$.

%The other families of generalised distortion conditions extend \ref{distortion_basic}) to range over some complex neighbourhood of the domain $\Lambda$.
Our second family of distortion conditions extend (\ref{distortion_basic}) to hold over an analytic neighbourhood of $\Lambda$. % and we define different distortion conditions specific to these two cases. 
For periodic intervals, the neighbourhood is the closed complex strip
$\Lambda^\beta_\delta = \{x+iy \mid  x \in [0,2\beta\pi], |y| \leq \delta\},$
 for a given $\delta > 0$, on which $v'$ is assumed to be holomorphic. For non-periodic intervals, the neighbourhood is $\check{\Lambda}_\delta$, defined to be a Bernstein ellipse\footnote{A Bernstein ellipse of parameter $\rho>1$ is an ellipse in the complex plane centred at $0$ with semi-major axis of length $\frac{1}{2}(\rho + \rho^{-1})$ along the real line and semi-minor axis $\frac{1}{2}(\rho - \rho^{-1})$.} of parameter $e^{\delta}$, on which the $v_\iota$ are assumed to be holomorphic. 
 
 The distortion condition itself is that
\begin{equation} %\sup_{x\in\Lambda_\delta} |v'(x)| \leq 1 \ 
\begin{cases}\sup_{z\in\Lambda^\beta_\delta}\left|\frac{v''(z)}{v'(z)}\right| = C_{1,\delta} < \infty,& \Lambda = [0,2\pi),\\
\sup_{\iota\in I,z\in \check{\Lambda}_\delta}\left|\frac{v_\iota''(z)}{v_\iota'(z)}\right| = C_{1,\delta} < \infty,& \Lambda = [-1,1].
\end{cases}
 \label{distortion_ana}\tag{$\DA_\delta$}\end{equation}
If no stipulation is put on $C_{1,\delta}$, this distortion condition for a periodic (respectively a finite-branched non-periodic map) is satisfied simply if $v' \neq 0$ on $\Lambda^\beta_\delta$ (resp. $v_\iota'\neq 0$ on $\check{\Lambda}_\delta$).
%\begin{equation}\sup_{x\in[0,2\beta\pi]}\left|(\log v')'(x+i\delta)\right| = C_{1,\delta} < \infty,\label{distortion_ana_four}\tag{$A_\delta^F$}.\end{equation}

%For non-periodic domains our distortion condition assumes that for a given $\delta > 0$, the branch inverses $v_\iota$ are holomorphic on and inside $\check{\Lambda}_\delta$, the Bernstein ellipse of parameter $e^{\delta}$, and requires that
%\begin{equation} %\sup_{\iota\in I,x\in \check{\Lambda}_\delta}\sqrt{\frac{1-x^2}{1-v_\iota(x)^2}}\left|v_\iota'(x)\right| \leq 1,\ 
%\sup_{\iota\in I,z\in \check{\Lambda}_\delta}\left|\frac{v_\iota''(z)}{v_\iota'(z)}\right| = C_{1,\delta} < \infty.\label{distortion_ana_cheb}\tag{A$_\delta^C$}\end{equation}

To succinctly formulate the main theorems in the next section, we will associate to these distortion conditions {\it standard spectral rates of convergence}. We define these rates of convergence $\kappa(\cdot)$ as function classes:
\begin{equation} \kappa\left(\DD_{r}\right) = \left\{ x \mapsto C (1+x)^{-r} : C > 0\right\},  \label{spectral_rate_diff}\end{equation}
\begin{equation} \kappa\left(\DA_{\delta}\right) = \left\{x \mapsto C e^{-\zeta x} : C > 0,\ \zeta \in (0,\delta] \right\}. \label{spectral_rate_ana}\end{equation}



%Choices include Lipschitz spaces \cite{MelbourneLectures}, fractional Sobolev spaces \cite{Baladi09,Thomine11,BaladiZetaBook}, and spaces of bounded variation \cite{Galatolo14, Liverani04}. If appropriate distortion conditions are satisfied, they may additionally have spectral gaps in various differentiability spaces \cite{BaladiBook}, Sobolev spaces \cite{Liverani01, BaladiZetaBook}, and Hardy spaces on $\Lambda_\delta$ or $\check{\Lambda}_\delta$.

